Investigating Practices and Opportunities for Cross-functional Collaboration around AI Fairness in Industry Practice

An emerging body of research indicates that ineffective cross-functional collaboration -- the interdisciplinary work done by industry practitioners across roles -- represents a major barrier to addressing issues of fairness in AI design and development. In this research, we sought to better understand practitioners' current practices and tactics to enact cross-functional collaboration for AI fairness, in order to identify opportunities to support more effective collaboration. We conducted a series of interviews and design workshops with 23 industry practitioners spanning various roles from 17 companies. We found that practitioners engaged in bridging work to overcome frictions in understanding, contextualization, and evaluation around AI fairness across roles. In addition, in organizational contexts with a lack of resources and incentives for fairness work, practitioners often piggybacked on existing requirements (e.g., for privacy assessments) and AI development norms (e.g., the use of quantitative evaluation metrics), although they worry that these tactics may be fundamentally compromised. Finally, we draw attention to the invisible labor that practitioners take on as part of this bridging and piggybacking work to enact interdisciplinary collaboration for fairness. We close by discussing opportunities for both FAccT researchers and AI practitioners to better support cross-functional collaboration for fairness in the design and development of AI systems.

==> citation_prev.tex <==

@article{campbell2020purposive,
title={Purposive sampling: complex or simple? Research case examples},
author={Campbell, Steve and Greenwood, Melanie and Prior, Sarah and Shearer, Toniele and Walkem, Kerrie and Young, Sarah and Bywaters, Danielle and Walker, Kim},
journal={Journal of research in Nursing},
volume={25},
number={8},
pages={652--661},
year={2020},
publisher={SAGE Publications Sage UK: London, England}
}

@article{rakova2021responsible,
  title={Where responsible AI meets reality: Practitioner perspectives on enablers for shifting organizational practices},
  author={Rakova, Bogdana and Yang, Jingying and Cramer, Henriette and Chowdhury, Rumman},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={5},
  number={CSCW1},
  pages={1--23},
  year={2021},
  publisher={ACM New York, NY, USA}
}



@inproceedings{shen2022model,
  title={The Model Card Authoring Toolkit: Toward Community-centered, Deliberation-driven AI Design},
  author={Shen, Hong and Wang, Leijie and Deng, Wesley H and Brusse, Ciell and Velgersdijk, Ronald and Zhu, Haiyi},
  booktitle={2022 ACM Conference on Fairness, Accountability, and Transparency},
  pages={440--451},
  year={2022}
}

@inproceedings{deng_2022_beyond,
author = {Mehandru, Nikita and Robertson, Samantha and Salehi, Niloufar},
title = {Beyond General Purpose Machine Translation: The Need for Context-specific Empirical Research to Design for Appropriate User Trust},
year = {2022},
isbn = {},
publisher = {},
address = {},
url = {},
doi = {},
abstract = {},
booktitle = {Workshop on Trust and Reliance in AI-Human Teams at CHI 2022},
articleno = {},
numpages = {},
keywords = {},
location = {},
series = {TRAIT 2022}
}

@inproceedings{robertson2020-what,
  title={What If I Don't Like Any Of The Choices? The Limits of Preference Elicitation for Participatory Algorithm Design},
  author={Robertson, Samantha and Salehi, Niloufar},
  booktitle={Workshop on Participatory Approaches to Machine Learning at ICML 2020},
  year={2020}
}

@inproceedings{robertson2021-three,
  title={Three Directions for the Design of Human-Centered Machine Translation},
  author={Samantha Robertson, Wesley Hanwen Deng, Timnit Gebru, Margaret Mitchell, Daniel J. Liebling, Michal Lahav, Katherine Heller, Mark Díaz, Samy Bengio, Niloufar Salehi},
  booktitle={HCI + MT Workshop at EACL '21},
  year={2021}
}

@inproceedings{mitchell2019model,
  title={Model cards for model reporting},
  author={Mitchell, Margaret and Wu, Simone and Zaldivar, Andrew and Barnes, Parker and Vasserman, Lucy and Hutchinson, Ben and Spitzer, Elena and Raji, Inioluwa Deborah and Gebru, Timnit},
  booktitle={Proceedings of the conference on fairness, accountability, and transparency},
  pages={220--229},
  year={2019}
}

@article{varshney2019trustworthy,
  title={Trustworthy machine learning and artificial intelligence},
  author={Varshney, Kush R},
  journal={XRDS: Crossroads, The ACM Magazine for Students},
  volume={25},
  number={3},
  pages={26--29},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{hossain2012users,
  title={Users' motivation to participate in online crowdsourcing platforms},
  author={Hossain, Mokter},
  booktitle={2012 International Conference on Innovation Management and Technology Research},
  pages={310--315},
  year={2012},
  organization={IEEE}
}


% Guidelines and toolkits

@article{googlePAIR,
title={People AI Guidebook},
url={https://pair.withgoogle.com/guidebook/}, author = {People + AI Research},
year={2021}}

@misc{openAI,
title={OpenAI: Our approach to alignment research},
url={https://openai.com/blog/our-approach-to-alignment-research/}, author = {OpenAI}
year={2022}, month = {August}}

@article{AIX360API,
title={AIX360 API},
url={https://aix360.mybluemix.net/}, author = {IBM Resaerch Trusted AI}, year={2021}}

@article{AIF360API,
title={AIF360 API},
url={https://aif360.mybluemix.net/}, author = {IBM Resaerch Trusted AI},
year={2021}}

@misc{ChatGPT,
title={Open AI, ChatGPT},
url={https://openai.com/blog/chatgpt/}, author = {OpenAI}
year={2022}, month={November}}

@misc{HuggingFace,
title={HuggingFace announcedthe new feature to flag any Model, Dataset, or Space on the Hub},
url={https://twitter.com/GiadaPistilli/status/1571865167092396033?s=20&t=LRhhEu63s6ftPmtZdfz8Cw}, author = {Pistilli, Giada},
year={2022}, month={September}}

@misc{ChatGPT_Feedback, title={ChatGPT Feedback Contest: Official Rules}, url={https://cdn.openai.com/chatgpt/ChatGPT_Feedback_Contest_Rules.pdf}, journal={Open AI}, author={Open AI}, year={2022}, month={December}} 


@misc{LaMDA, title={LaMDA: our breakthrough conversation technology}, url={https://blog.google/technology/ai/lamda/}, journal={Google}, author={Collins, Eli and Ghahramani, Zoubin}, year={2021}, month={May}} 

@misc{Facebook_Ban, title={Facebook forced to ban its AI after it ‘revealed how to make napalm and made racist comments}, url={https://www.the-sun.com/tech/6729391/meta-withdraws-ai-galactica-controversy/}, journal={The U.S Sun}, author = {Harris, Jamie},
year={2022}, month={November}} 

@misc{Tay_Ban,
title={Microsoft’s Racist Chatbot Revealed the Dangers of Online Conversation The bot learned language from people on Twitter—but it also learned values},
url={https://spectrum.ieee.org/in-2016-microsofts-racist-chatbot-revealed-the-dangers-of-online-conversation}, journal = {Spectrum}, author = {Schwartz, Oscar},
year={2019}, month={November}}

@misc{AItest,
  title = {AI Test Kitchen},
  author = {Warkentin, Tris and Woodward, Josh},
  url = {https://blog.google/technology/ai/join-us-in-the-ai-test-kitchen/},
  year={2022}}

@misc{MSRchecklist,
  author = {Microsoft Research},
  title =  {AI Fairness Checklist},
  url = {https://blog.google/technology/ai/join-us-in-the-ai-test-kitchen/},
  year = {2022}
}

@misc{FairlearnAPI,
  author = {Sarah Bird},
  title =  {Fairlearn API},
  url = {https://fairlearn.github.io/v0.5.0/api_reference/fairlearn.datasets.html},
  year = {2020}
}

@article{bellamy2018ai,
  title={AI Fairness 360: An extensible toolkit for detecting and mitigating algorithmic bias},
  author={Bellamy, Rachel KE and Dey, Kuntal and Hind, Michael and Hoffman, Samuel C and Houde, Stephanie and Kannan, Kalapriya and Lohia, Pranay and Martino, Jacquelyn and Mehta, Sameep and Mojsilovi{\'c}, Aleksandra and others},
  journal={IBM Journal of Research and Development},
  volume={63},
  number={4/5},
  pages={4--1},
  year={2019},
  publisher={IBM}
}

@techreport{bird2020fairlearn,
author = {Bird, Sarah and Dudík, Miro and Edgar, Richard and Horn, Brandon and Lutz, Roman and Milan, Vanessa and Sameki, Mehrnoosh and Wallach, Hanna and Walker, Kathleen},
title = {Fairlearn: A toolkit for assessing and improving fairness in AI},
institution = {Microsoft},
year = {2020},
month = {May},
abstract = {We introduce Fairlearn, an open source toolkit that empowers data scientists and developers to assess and improve the fairness of their AI systems. Fairlearn has two components: an interactive visualization dashboard and unfairness mitigation algorithms. These components are designed to help with navigating trade-offs between fairness and model performance. We emphasize that prioritizing fairness in AI systems is a sociotechnical challenge. Because there are many complex sources of unfairness—some societal and some technical—it is not possible to fully “debias” a system or to guarantee fairness; the goal is to mitigate fairness-related harms as much as possible. As Fairlearn grows to include additional fairness metrics, unfairness mitigation algorithms, and visualization capabilities, we hope that it will be shaped by a diverse community of stakeholders, ranging from data scientists, developers, and business decision makers to the people whose lives may be affected by the predictions of AI systems.},
url = {https://www.microsoft.com/en-us/research/publication/fairlearn-a-toolkit-for-assessing-and-improving-fairness-in-ai/},
number = {MSR-TR-2020-32},
}

@article{malladi2019bug,
title={Bug bounty programs for cybersecurity: Practices, issues, and recommendations},
author={Malladi, Suresh S and Subramanian, Hemang C},
journal={IEEE Software},
volume={37},
number={1},
pages={31--39},
year={2019},
publisher={IEEE}
}

@article{chowdhury2021introducing,
title={Introducing Twitter’s first algorithmic bias bounty challenge},
author={Chowdhury, Rumman and Williams, Jutta},
journal={URl: https://blog. twitter. com/engineering/en\_us/topics/insights/2021/algorithmic-bias-bountychallenge},
year={2021}
}

@inproceedings{raji2022outsider,
title={Outsider Oversight: Designing a Third Party Audit Ecosystem for AI Governance},
author={Raji, Inioluwa Deborah and Xu, Peggy and Honigsberg, Colleen and Ho, Daniel},
booktitle={Proceedings of the 2022 AAAI/ACM Conference on AI, Ethics, and Society},
pages={557--571},
year={2022}
}


@inproceedings{gordon2022jury,
  title={Jury learning: Integrating dissenting voices into machine learning models},
  author={Gordon, Mitchell L and Lam, Michelle S and Park, Joon Sung and Patel, Kayur and Hancock, Jeff and Hashimoto, Tatsunori and Bernstein, Michael S},
  booktitle={CHI Conference on Human Factors in Computing Systems},
  pages={1--19},
  year={2022}
}

@article{chowdhury2021introducing,
  title={Introducing Twitter’s first algorithmic bias bounty challenge},
  author={Chowdhury, Rumman and Williams, Jutta},
  journal={URl: https://blog. twitter. com/engineering/en\_us/topics/insights/2021/algorithmic-bias-bountychallenge},
  year={2021}
}

@article{vaughan2017making,
  title={Making Better Use of the Crowd: How Crowdsourcing Can Advance Machine Learning Research.},
  author={Vaughan, Jennifer Wortman},
  journal={J. Mach. Learn. Res.},
  volume={18},
  number={1},
  pages={7026--7071},
  year={2017}
}

@inproceedings{steiger2021psychological,
  title={The psychological well-being of content moderators: the emotional labor of commercial moderation and avenues for improving support},
  author={Steiger, Miriah and Bharucha, Timir J and Venkatagiri, Sukrit and Riedl, Martin J and Lease, Matthew},
  booktitle={Proceedings of the 2021 CHI conference on human factors in computing systems},
  pages={1--14},
  year={2021}
}

@article{young2019toward,
  title={Toward inclusive tech policy design: a method for underrepresented voices to strengthen tech policy documents},
  author={Young, Meg and Magassa, Lassana and Friedman, Batya},
  journal={Ethics and Information Technology},
  volume={21},
  number={2},
  pages={89--103},
  year={2019},
  publisher={Springer}
}

@article{braun2019reflecting,
  title={Reflecting on reflexive thematic analysis},
  author={Braun, Virginia and Clarke, Victoria},
  journal={Qualitative research in sport, exercise and health},
  volume={11},
  number={4},
  pages={589--597},
  year={2019},
  publisher={Taylor \& Francis}
}
 
@article{kraut2011encouraging,
  title={Encouraging contribution to online communities},
  author={Kraut, Robert E and Resnick, Paul},
  journal={Building successful online communities: Evidence-based social design},
  pages={21--76},
  year={2011},
  publisher={MIT Press Cambridge, MA}
}


@inproceedings{dosono2019moderation,
  title={Moderation practices as emotional labor in sustaining online communities: The case of AAPI identity work on Reddit},
  author={Dosono, Bryan and Semaan, Bryan},
  booktitle={Proceedings of the 2019 CHI conference on human factors in computing systems},
  pages={1--13},
  year={2019}
}

@article{ling2005using,
  title={Using social psychology to motivate contributions to online communities},
  author={Ling, Kimberly and Beenen, Gerard and Ludford, Pamela and Wang, Xiaoqing and Chang, Klarissa and Li, Xin and Cosley, Dan and Frankowski, Dan and Terveen, Loren and Rashid, Al Mamunur and others},
  journal={Journal of Computer-Mediated Communication},
  volume={10},
  number={4},
  pages={00--00},
  year={2005},
  publisher={Wiley Online Library}
}

@inproceedings{salehi2015we,
  title={We are dynamo: Overcoming stalling and friction in collective action for crowd workers},
  author={Salehi, Niloufar and Irani, Lilly C and Bernstein, Michael S and Alkhatib, Ali and Ogbe, Eva and Milland, Kristy},
  booktitle={Proceedings of the 33rd annual ACM conference on human factors in computing systems},
  pages={1621--1630},
  year={2015}
}

@article{metaxa2021auditing,
title={Auditing algorithms: Understanding algorithmic systems from the outside in},
author={Metaxa, Dana{\"e} and Park, Joon Sung and Robertson, Ronald E and Karahalios, Karrie and Wilson, Christo and Hancock, Jeff and Sandvig, Christian and others},
journal={Foundations and Trends{\textregistered} in Human--Computer Interaction},
volume={14},
number={4},
pages={272--344},
year={2021},
publisher={Now Publishers, Inc.}
}

@article{wang2022towards,
  title={Towards Intersectionality in Machine Learning: Including More Identities, Handling Underrepresentation, and Performing Evaluation},
  author={Wang, Angelina and Ramaswamy, Vikram V and Russakovsky, Olga},
  journal={arXiv preprint arXiv:2205.04610},
  year={2022}
}

@article{lam2022enduser,
    author = {Lam, Michelle S. and Gordon, Mitchell L. and Metaxa, Dana\"{e} and Hancock, Jeffrey T. and Landay, James A. and Bernstein, Michael S.},
    title = {End-User Audits: A System Empowering Communities to Lead Large-Scale Investigations of Harmful Algorithmic Behavior},
    year = {2022},
    issue_date = {November 2022},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    volume = {6},
    number = {CSCW2},
    url = {https://doi.org/10.1145/3555625},
    doi = {10.1145/3555625},
    journal = {Proc. ACM Hum.-Comput. Interact.},
    month = {Nov},
    articleno = {512},
    numpages = {34}
}

@inproceedings{irani2013turkopticon,
  title={Turkopticon: Interrupting worker invisibility in amazon mechanical turk},
  author={Irani, Lilly C and Silberman, M Six},
  booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
  pages={611--620},
  year={2013}
}

@inproceedings{chen2019fairness,
title={Fairness under unawareness: Assessing disparity when protected class is unobserved},
author={Chen, Jiahao and Kallus, Nathan and Mao, Xiaojie and Svacha, Geoffry and Udell, Madeleine},
booktitle={Proceedings of the conference on fairness, accountability, and transparency},
pages={339--348},
year={2019}
}

@article{veale2017fairer,
title={Fairer machine learning in the real world: Mitigating discrimination without collecting sensitive data},
author={Veale, Michael and Binns, Reuben},
journal={Big Data \& Society},
volume={4},
number={2},
pages={2053951717743530},
year={2017},
publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{crawford2017trouble,
title={The trouble with bias},
author={Crawford, Kate},
booktitle={Conference on Neural Information Processing Systems, invited speaker},
year={2017}
}

@inproceedings{kaur2020interpreting,
  title={Interpreting interpretability: understanding data scientists' use of interpretability tools for machine learning},
  author={Kaur, Harmanpreet and Nori, Harsha and Jenkins, Samuel and Caruana, Rich and Wallach, Hanna and Wortman Vaughan, Jennifer},
  booktitle={Proceedings of the 2020 CHI conference on human factors in computing systems},
  pages={1--14},
  year={2020}
}

@article{cabrera2022did,
  title={What Did My AI Learn? How Data Scientists Make Sense of Model Behavior},
  author={Cabrera, {\'A}ngel Alexander and Ribeiro, Marco Tulio and Lee, Bongshin and DeLine, Rob and Perer, Adam and Drucker, Steven M},
  journal={ACM Transactions on Computer-Human Interaction},
  year={2022},
  publisher={ACM New York, NY}
}

@inproceedings{alkhatib2019street,
  title={Street-level algorithms: A theory at the gaps between policy and decisions},
  author={Alkhatib, Ali and Bernstein, Michael},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2019}
}

@article{evenson2006directed,
  title={Directed storytelling: Interpreting experience for design},
  author={Evenson, Shelley},
  journal={Design Studies: Theory and research in graphic design},
  pages={231--240},
  year={2006}
}

@inproceedings{holstein2019designing,
title={Designing for complementarity: Teacher and student needs for orchestration support in AI-enhanced classrooms},
author={Holstein, Kenneth and McLaren, Bruce M and Aleven, Vincent},
booktitle={International conference on artificial intelligence in education},
pages={157--171},
year={2019},
organization={Springer}
}

@inproceedings{nushi2018towards,
title={Towards accountable ai: Hybrid human-machine analyses for characterizing system failure},
author={Nushi, Besmira and Kamar, Ece and Horvitz, Eric},
booktitle={Proceedings of the AAAI Conference on Human Computation and Crowdsourcing},
volume={6},
pages={126--135},
year={2018}
}

@inproceedings{ochigame2021search,
title={Search Atlas: Visualizing Divergent Search Results Across Geopolitical Borders},
author={Ochigame, Rodrigo and Ye, Katherine},
booktitle={Designing Interactive Systems Conference 2021},
pages={1970--1983},
year={2021}
}

@article{passi2018trust,
  title={Trust in data science: Collaboration, translation, and accountability in corporate data science projects},
  author={Passi, Samir and Jackson, Steven J},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={2},
  number={CSCW},
  pages={1--28},
  year={2018},
  publisher={ACM New York, NY, USA}
}


@inproceedings{lee2021landscape,
  title={The landscape and gaps in open source fairness toolkits},
  author={Lee, Michelle Seng Ah and Singh, Jat},
  booktitle={Proceedings of the 2021 CHI conference on human factors in computing systems},
  pages={1--13},
  year={2021}
}

@inproceedings{attenberg2011beat,
  title={Beat the machine: Challenging workers to find the unknown unknowns},
  author={Attenberg, Josh M and Ipeirotis, Pagagiotis G and Provost, Foster},
  booktitle={Workshops at the Twenty-Fifth AAAI Conference on Artificial Intelligence},
  year={2011}
}

@article{kiela2021dynabench,
  title={Dynabench: Rethinking benchmarking in NLP},
  author={Kiela, Douwe and Bartolo, Max and Nie, Yixin and Kaushik, Divyansh and Geiger, Atticus and Wu, Zhengxuan and Vidgen, Bertie and Prasad, Grusha and Singh, Amanpreet and Ringshia, Pratik and others},
  journal={arXiv preprint arXiv:2104.14337},
  year={2021}
}

@article{holstein2019co,
 title={Designing for complementarity: Teacher and student needs for orchestration support in AI-enhanced classrooms},
  author={Holstein, Kenneth and McLaren, Bruce M and Aleven, Vincent},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={157--171},
  year={2019},
  organization={Springer}
}

@inproceedings{crawford2017trouble,
title={The trouble with bias},
author={Crawford, Kate},
booktitle={Conference on Neural Information Processing Systems, invited speaker},
year={2017}
}

@inproceedings{kaur2020interpreting,
  title={Interpreting interpretability: understanding data scientists' use of interpretability tools for machine learning},
  author={Kaur, Harmanpreet and Nori, Harsha and Jenkins, Samuel and Caruana, Rich and Wallach, Hanna and Wortman Vaughan, Jennifer},
  booktitle={Proceedings of the 2020 CHI conference on human factors in computing systems},
  pages={1--14},
  year={2020}
}

@article{cabrera2022did,
  title={What Did My AI Learn? How Data Scientists Make Sense of Model Behavior},
  author={Cabrera, {\'A}ngel Alexander and Ribeiro, Marco Tulio and Lee, Bongshin and DeLine, Rob and Perer, Adam and Drucker, Steven M},
  journal={ACM Transactions on Computer-Human Interaction},
  year={2022},
  publisher={ACM New York, NY}
}

@inproceedings{alkhatib2019street,
  title={Street-level algorithms: A theory at the gaps between policy and decisions},
  author={Alkhatib, Ali and Bernstein, Michael},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2019}
}

@article{harrington2019deconstructing,
  title={Deconstructing community-based collaborative design: Towards more equitable participatory design engagements},
  author={Harrington, Christina and Erete, Sheena and Piper, Anne Marie},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={3},
  number={CSCW},
  pages={1--25},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{raji2020closing,
  title={Closing the AI accountability gap: Defining an end-to-end framework for internal algorithmic auditing},
  author={Raji, Inioluwa Deborah and Smart, Andrew and White, Rebecca N and Mitchell, Margaret and Gebru, Timnit and Hutchinson, Ben and Smith-Loud, Jamila and Theron, Daniel and Barnes, Parker},
  booktitle={Proceedings of the 2020 conference on fairness, accountability, and transparency},
  pages={33--44},
  year={2020}
}

@article{groce2013you,
  title={You are the only possible oracle: Effective test selection for end users of interactive machine learning systems},
  author={Groce, Alex and Kulesza, Todd and Zhang, Chaoqiang and Shamasunder, Shalini and Burnett, Margaret and Wong, Weng-Keen and Stumpf, Simone and Das, Shubhomoy and Shinsel, Amber and Bice, Forrest and others},
  journal={IEEE Transactions on Software Engineering},
  volume={40},
  number={3},
  pages={307--323},
  year={2013},
  publisher={IEEE}
}

@inproceedings{wu2019errudite,
  title={Errudite: Scalable, reproducible, and testable error analysis},
  author={Wu, Tongshuang and Ribeiro, Marco Tulio and Heer, Jeffrey and Weld, Daniel S},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={747--763},
  year={2019}
}

@article{sloane2020participation,
  title={Participation is not a design fix for machine learning},
  author={Sloane, Mona and Moss, Emanuel and Awomolo, Olaitan and Forlano, Laura},
  journal={arXiv preprint arXiv:2007.02423},
  year={2020}
}

@article{hsu2022empowering,
  title={Empowering local communities using artificial intelligence},
  author={Hsu, Yen-Chia and Verma, Himanshu and Mauri, Andrea and Nourbakhsh, Illah and Bozzon, Alessandro and others},
  journal={Patterns},
  volume={3},
  number={3},
  pages={100449},
  year={2022},
  publisher={Elsevier}
}

@article{evenson2006directed,
  title={Directed storytelling: Interpreting experience for design},
  author={Evenson, Shelley},
  journal={Design Studies: Theory and research in graphic design},
  pages={231--240},
  year={2006}
}

@inproceedings{holstein2019designing,
title={Designing for complementarity: Teacher and student needs for orchestration support in AI-enhanced classrooms},
author={Holstein, Kenneth and McLaren, Bruce M and Aleven, Vincent},
booktitle={International conference on artificial intelligence in education},
pages={157--171},
year={2019},
organization={Springer}
}

@article{attenberg2015beat,
  title={Beat the machine: Challenging humans to find a predictive model's “unknown unknowns”},
  author={Attenberg, Joshua and Ipeirotis, Panos and Provost, Foster},
  journal={Journal of Data and Information Quality (JDIQ)},
  volume={6},
  number={1},
  pages={1--17},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@article{evenson2006directed,
  title={Directed storytelling: Interpreting experience for design},
  author={Evenson, Shelley},
  journal={Design Studies: Theory and research in graphic design},
  pages={231--240},
  year={2006}
}

@inproceedings{deng2022exploring,
	address = {Seoul Republic of Korea},
	title = {Exploring {How} {Machine} {Learning} {Practitioners} ({Try} {To}) {Use} {Fairness} {Toolkits}},
	isbn = {978-1-4503-9352-2},
	url = {https://dl.acm.org/doi/10.1145/3531146.3533113},
	doi = {10.1145/3531146.3533113},
	language = {en},
	urldate = {2022-08-10},
	booktitle = {2022 {ACM} {Conference} on {Fairness}, {Accountability}, and {Transparency}},
	publisher = {ACM},
	author = {Deng, Wesley Hanwen and Nagireddy, Manish and Lee, Michelle Seng Ah and Singh, Jatinder and Wu, Zhiwei Steven and Holstein, Kenneth and Zhu, Haiyi},
	month = jun,
	year = {2022},
	pages = {473--484},
}

@article{cramer2018assessing,
  title={Assessing and addressing algorithmic bias in practice},
  author={Cramer, Henriette and Garcia-Gathright, Jean and Springer, Aaron and Reddy, Sravana},
  journal={Interactions},
  volume={25},
  number={6},
  pages={58--63},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@inproceedings{richardson2021towards,
  title={Towards Fairness in Practice: A Practitioner-Oriented Rubric for Evaluating Fair ML Toolkits},
  author={Richardson, Brianna and Garcia-Gathright, Jean and Way, Samuel F and Thom, Jennifer and Cramer, Henriette},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2021}
}

@article{madaio2021assessing,
  title={Assessing the Fairness of AI Systems: AI Practitioners' Processes, Challenges, and Needs for Support},
  author={Madaio, Michael and Egede, Lisa and Subramonyam, Hariharan and Vaughan, Jennifer Wortman and Wallach, Hanna},
  journal={arXiv preprint arXiv:2112.05675},
  year={2021}
}

@article{liang_advances_2022,
	title = {Advances, challenges and opportunities in creating data for trustworthy {AI}},
	issn = {2522-5839},
	url = {https://www.nature.com/articles/s42256-022-00516-1},
	doi = {10.1038/s42256-022-00516-1},
	language = {en},
	urldate = {2022-08-26},
	journal = {Nature Machine Intelligence},
	author = {Liang, Weixin and Tadesse, Girmaw Abebe and Ho, Daniel and Li, Fei-Fei and Zaharia, Matei and Zhang, Ce and Zou, James},
	month = aug,
	year = {2022},
}

@inproceedings{callison2010creating,
  title={Creating speech and language data with amazon’s mechanical turk},
  author={Callison-Burch, Chris and Dredze, Mark},
  booktitle={Proceedings of the NAACL HLT 2010 workshop on creating speech and language data with Amazon’s Mechanical Turk},
  pages={1--12},
  year={2010}
}

@inproceedings{snow2008cheap,
  title={Cheap and fast--but is it good? evaluating non-expert annotations for natural language tasks},
  author={Snow, Rion and O’connor, Brendan and Jurafsky, Dan and Ng, Andrew Y},
  booktitle={Proceedings of the 2008 conference on empirical methods in natural language processing},
  pages={254--263},
  year={2008}
}

@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@inproceedings{zaidan2011crowdsourcing,
  title={Crowdsourcing translation: Professional quality from non-professionals},
  author={Zaidan, Omar and Callison-Burch, Chris},
  booktitle={Proceedings of the 49th annual meeting of the association for computational linguistics: human language technologies},
  pages={1220--1229},
  year={2011}
}

@article{zhou2019hype,
  title={Hype: A benchmark for human eye perceptual evaluation of generative models},
  author={Zhou, Sharon and Gordon, Mitchell and Krishna, Ranjay and Narcomey, Austin and Fei-Fei, Li F and Bernstein, Michael},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@article{anastasiou2011comparison,
  title={Comparison of crowdsourcing translation with Machine Translation},
  author={Anastasiou, Dimitra and Gupta, Rajat},
  journal={Journal of Information Science},
  volume={37},
  number={6},
  pages={637--659},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}

@article{kroll2016accountable,
  title={Accountable algorithms},
  author={Kroll, Joshua A and Barocas, Solon and Felten, Edward W and Reidenberg, Joel R and Robinson, David G and Yu, Harlan},
  journal={U. Pa. L. Rev.},
  volume={165},
  pages={633},
  year={2016},
  publisher={HeinOnline}
}

@inproceedings{abebe2020roles,
  title={Roles for computing in social change},
  author={Abebe, Rediet and Barocas, Solon and Kleinberg, Jon and Levy, Karen and Raghavan, Manish and Robinson, David G},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
  pages={252--260},
  year={2020}
}

"@article{hsu2021empowering,
  title={Empowering Local Communities Using Artificial Intelligence},
  author={Hsu, Yen-Chia and Huang, Ting-Hao'Kenneth' and Verma, Himanshu and Mauri, Andrea and Nourbakhsh, Illah and Bozzon, Alessandro},
  journal={arXiv preprint arXiv:2110.02007},
  year={2021}
}"

@inproceedings{costanza2022audits,
  title={Who Audits the Auditors? Recommendations from a field scan of the algorithmic auditing ecosystem},
  author={Costanza-Chock, Sasha and Raji, Inioluwa Deborah and Buolamwini, Joy},
  booktitle={2022 ACM Conference on Fairness, Accountability, and Transparency},
  pages={1571--1583},
  year={2022}
}

@article{DeVos2022TowardUA,
  title={Toward User-Driven Algorithm Auditing: Investigating users’ strategies for uncovering harmful algorithmic behavior},
  author={Alicia DeVos and Aditi Dhabalia and Hong Shen and Kenneth Holstein and Motahhare Eslami},
  journal={CHI Conference on Human Factors in Computing Systems},
  year={2022}
}

%Crowdsourcing

@inproceedings{kittur2013future,
  title={The future of crowd work},
  author={Kittur, Aniket and Nickerson, Jeffrey V and Bernstein, Michael and Gerber, Elizabeth and Shaw, Aaron and Zimmerman, John and Lease, Matt and Horton, John},
  booktitle={Proceedings of the 2013 conference on Computer supported cooperative work},
  pages={1301--1318},
  year={2013}
}

@article{bigham2015human,
  title={Human-computer interaction and collective intelligence},
  author={Bigham, Jeffrey P and Bernstein, Michael S and Adar, Eytan},
  journal={Handbook of collective intelligence},
  volume={57},
  year={2015},
  publisher={Mit Press Cambridge, MA, USA}
}

@inproceedings{bernstein2011crowds,
  title={Crowds in two seconds: Enabling realtime crowd-powered interfaces},
  author={Bernstein, Michael S and Brandt, Joel and Miller, Robert C and Karger, David R},
  booktitle={Proceedings of the 24th annual ACM symposium on User interface software and technology},
  pages={33--42},
  year={2011}
}

@inproceedings{dekel2009vox,
  title={Vox Populi: Collecting High-Quality Labels from a Crowd.},
  author={Dekel, Ofer and Shamir, Ohad},
  booktitle={COLT},
  year={2009}
}

@InProceedings{pmlr-v80-kilbertus18a,
  title = 	 {Blind Justice: Fairness with Encrypted Sensitive Attributes},
  author =       {Kilbertus, Niki and Gascon, Adria and Kusner, Matt and Veale, Michael and Gummadi, Krishna and Weller, Adrian},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {2630--2639},
  year = 	 {2018},
  editor = 	 {Dy, Jennifer and Krause, Andreas},
  volume = 	 {80},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {10--15 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v80/kilbertus18a/kilbertus18a.pdf},
  url = 	 {https://proceedings.mlr.press/v80/kilbertus18a.html},
  abstract = 	 {Recent work has explored how to train machine learning models which do not discriminate against any subgroup of the population as determined by sensitive attributes such as gender or race. To avoid disparate treatment, sensitive attributes should not be considered. On the other hand, in order to avoid disparate impact, sensitive attributes must be examined, e.g., in order to learn a fair model, or to check if a given model is fair. We introduce methods from secure multi-party computation which allow us to avoid both. By encrypting sensitive attributes, we show how an outcome-based fair model may be learned, checked, or have its outputs verified and held to account, without users revealing their sensitive attributes.}
}

@article{mcdonald2019reliability,
  title={Reliability and inter-rater reliability in qualitative research: Norms and guidelines for CSCW and HCI practice},
  author={McDonald, Nora and Schoenebeck, Sarita and Forte, Andrea},
  journal={Proceedings of the ACM on human-computer interaction},
  volume={3},
  number={CSCW},
  pages={1--23},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@inproceedings{robertson2020-what,
  title={What If I Don't Like Any Of The Choices? The Limits of Preference Elicitation for Participatory Algorithm Design},
  author={Robertson, Samantha and Salehi, Niloufar},
  booktitle={Workshop on Participatory Approaches to Machine Learning at ICML 2020},
  year={2020}
}

@inproceedings{raji2020saving,
  title={Saving face: Investigating the ethical concerns of facial recognition auditing},
  author={Raji, Inioluwa Deborah and Gebru, Timnit and Mitchell, Margaret and Buolamwini, Joy and Lee, Joonseok and Denton, Emily},
  booktitle={Proceedings of the AAAI/ACM Conference on AI, Ethics, and Society},
  pages={145--151},
  year={2020}
}

@article{Cramer2018AssessingAA,
  title={Assessing and addressing algorithmic bias in practice},
  author={Henriette Cramer and Jean I. Garcia-Gathright and Aaron Springer and Sravana Reddy},
  journal={Interactions},
  year={2018},
  volume={25},
  pages={58 - 63}
}

@article{Wallace2013MakingDP,
  title={Making design probes work},
  author={Jayne Wallace and John C. McCarthy and Peter C. Wright and Patrick Olivier},
  journal={Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
  year={2013}
}

@article{Sindlinger2010CrowdsourcingWT,
  title={Crowdsourcing: Why the Power of the Crowd is Driving the Future of Business},
  author={Ted S. Sindlinger},
  journal={American Journal of Health-system Pharmacy},
  year={2010},
  volume={67},
  pages={1565-1566}
}

@inproceedings{Bigham2014HumanComputerIA,
  title={Human-Computer Interaction and Collective Intelligence},
  author={Jeffrey P. Bigham and Michael S. Bernstein and Eytan Adar},
  year={2014}
}

@article{Bernstein2010SoylentAW,
  title={Soylent: a word processor with a crowd inside},
  author={Michael S. Bernstein and Greg Little and Rob Miller and Bj{\"o}rn Hartmann and Mark S. Ackerman and David R. Karger and David Crowell and Katrina Panovich},
  journal={Proceedings of the 23nd annual ACM symposium on User interface software and technology},
  year={2010}
}

@article{Young2019TowardIT,
  title={Toward inclusive tech policy design: a method for underrepresented voices to strengthen tech policy documents},
  author={Meg Young and Lassana Magassa and Batya Friedman},
  journal={Ethics and Information Technology},
  year={2019},
  volume={21},
  pages={89-103}
}

@inproceedings{irani2013turkopticon,
  title={Turkopticon: Interrupting worker invisibility in amazon mechanical turk},
  author={Irani, Lilly C and Silberman, M Six},
  booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
  pages={611--620},
  year={2013}
}

@article{metaxa2021auditing,
  title={Auditing algorithms: Understanding algorithmic systems from the outside in},
  author={Metaxa, Dana{\"e} and Park, Joon Sung and Robertson, Ronald E and Karahalios, Karrie and Wilson, Christo and Hancock, Jeff and Sandvig, Christian and others},
  journal={Foundations and Trends{\textregistered} in Human--Computer Interaction},
  volume={14},
  number={4},
  pages={272--344},
  year={2021},
  publisher={Now Publishers, Inc.}
}

@article{cscw2021-severus-qual,
  title = {A {Framework} of {Severity} for {Harmful} {Content} {Online}},
  volume = {5},
  number = {CSCW2},
  journal = {Proc. ACM Hum.-Comput. Interact.},
  author = {Scheuerman, Morgan Klaus and Jiang, Jialun Aaron and Fiesler, Casey and Brubaker, Jed R.},
  year = {2021},
  month = oct,
  pages = {Article 368},
  doi = {10.1145/3479512}
}

@article{chen2021goldilocks,
  title={Goldilocks: Consistent Crowdsourced Scalar Annotations with Relative Uncertainty},
  author={Chen, Quan Ze and Weld, Daniel S and Zhang, Amy X},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={5},
  number={CSCW2},
  pages={1--25},
  year={2021},
  publisher={ACM New York, NY, USA}
}


@article{toxtli2021quantifying,
  title={Quantifying the Invisible Labor in Crowd Work},
  author={Toxtli, Carlos and Suri, Siddharth and Savage, Saiph},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={5},
  number={CSCW2},
  pages={1--26},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@book{gray2019ghost,
  title={Ghost work: How to stop Silicon Valley from building a new global underclass},
  author={Gray, Mary L and Suri, Siddharth},
  year={2019},
  publisher={Eamon Dolan Books}
}

@article{Kittur2013TheFO,
  title={The future of crowd work},
  author={Aniket Kittur and Jeffrey V. Nickerson and Michael S. Bernstein and Elizabeth Gerber and Aaron D. Shaw and John Zimmerman and Matthew Lease and John Joseph Horton},
  journal={Proceedings of the 2013 conference on Computer supported cooperative work},
  year={2013}
}

@article{lease2013mechanical,
  title={Mechanical turk is not anonymous},
  author={Lease, Matthew and Hullman, Jessica and Bigham, Jeffrey and Bernstein, Michael and Kim, Juho and Lasecki, Walter and Bakhshi, Saeideh and Mitra, Tanushree and Miller, Robert},
  journal={Available at SSRN 2228728},
  year={2013}
}

@book{eubanks2018automating,
  title={Automating inequality: How high-tech tools profile, police, and punish the poor},
  author={Eubanks, Virginia},
  year={2018},
  publisher={St. Martin's Press}
}


@article{angwin2016machine,
  title={Machine bias},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  year={2016},
  journal={ProPublica},
  url={https://www.propublica.org/article/machine-bias-risk-assessments-in-criminal-sentencing},
  month=may
}

@article{barocas2016big,
  title={Big data's disparate impact},
  author={Barocas, Solon and Selbst, Andrew D},
  journal={Calif. L. Rev.},
  volume={104},
  pages={671},
  year={2016},
  publisher={HeinOnline}
}

@article{sandvig2014auditing,
  title={Auditing algorithms: Research methods for detecting discrimination on internet platforms},
  author={Sandvig, Christian and Hamilton, Kevin and Karahalios, Karrie and Langbort, Cedric},
  journal={Data and Discrimination: Converting Critical Concerns into Productive Inquiry},
  year={2014}
}

@book{noble2018algorithms,
  title={Algorithms of oppression: How search engines reinforce racism},
  author={Noble, Safiya Umoja},
  year={2018},
  publisher={NYU Press}
}

@inproceedings{hannak2014measuring,
  title={Measuring price discrimination and steering on e-commerce web sites},
  author={Hannak, Aniko and Soeller, Gary and Lazer, David and Mislove, Alan and Wilson, Christo},
  booktitle={Proceedings of the 2014 Conference on Internet Measurement Conference},
  pages={305--318},
  year={2014}
}

@inproceedings{eslami2017careful,
  title={“Be careful; things can be worse than they appear”: Understanding Biased Algorithms and Users’ Behavior around Them in Rating Platforms},
  author={Eslami, Motahhare and Vaccaro, Kristen and Karahalios, Karrie and Hamilton, Kevin},
  booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
  volume={11},
  number={1},
  year={2017}
}

@inproceedings{buolamwini2018gender,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on fairness, accountability and transparency},
  pages={77--91},
  year={2018},
  organization={PMLR}
}

@inproceedings{eslami2019user,
  title={User attitudes towards algorithmic opacity and transparency in online reviewing platforms},
  author={Eslami, Motahhare and Vaccaro, Kristen and Lee, Min Kyung and Elazari Bar On, Amit and Gilbert, Eric and Karahalios, Karrie},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--14},
  year={2019}
}



@inproceedings{asplund2020auditing,
title={Auditing race and gender discrimination in online housing markets},
author={Asplund, Joshua and Eslami, Motahhare and Sundaram, Hari and Sandvig, Christian and Karahalios, Karrie},
booktitle={Proceedings of the International AAAI Conference on Web and Social Media},
volume={14},
pages={24--35},
year={2020}
}

@inproceedings{raji2019actionable,
  title={Actionable auditing: Investigating the impact of publicly naming biased performance results of commercial AI products},
  author={Raji, Inioluwa Deborah and Buolamwini, Joy},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={429--435},
  year={2019}
}

@article{sweeney2013discrimination,
  title={Discrimination in online ad delivery},
  author={Sweeney, Latanya},
  journal={Queue},
  volume={11},
  number={3},
  pages={10--29},
  year={2013},
  publisher={ACM New York, NY, USA}
}

@article{prates2020assessing,
  title={Assessing gender bias in machine translation: a case study with google translate},
  author={Prates, Marcelo OR and Avelar, Pedro H and Lamb, Lu{\'\i}s C},
  journal={Neural Computing and Applications},
  volume={32},
  number={10},
  pages={6363--6381},
  year={2020},
  publisher={Springer}
}
@article{dow2010parallel,
  title={Parallel prototyping leads to better design results, more divergence, and increased self-efficacy},
  author={Dow, Steven P and Glassco, Alana and Kass, Jonathan and Schwarz, Melissa and Schwartz, Daniel L and Klemmer, Scott R},
  journal={ACM Transactions on Computer-Human Interaction (TOCHI)},
  volume={17},
  number={4},
  pages={1--24},
  year={2010},
  publisher={ACM New York, NY, USA}
}

@inproceedings{smith2022real,
  title={REAL ML: Recognizing, Exploring, and Articulating Limitations of Machine Learning Research},
  author={Smith, Jessie J and Amershi, Saleema and Barocas, Solon and Wallach, Hanna and Wortman Vaughan, Jennifer},
  booktitle={2022 ACM Conference on Fairness, Accountability, and Transparency},
  pages={587--597},
  year={2022}
}

@inproceedings{madaio2020co,
  title={Co-designing checklists to understand organizational challenges and opportunities around fairness in ai},
  author={Madaio, Michael A and Stark, Luke and Wortman Vaughan, Jennifer and Wallach, Hanna},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--14},
  year={2020}
}

@article{zhu2018value,
  title={Value-sensitive algorithm design: Method, case study, and lessons},
  author={Zhu, Haiyi and Yu, Bowen and Halfaker, Aaron and Terveen, Loren},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={2},
  number={CSCW},
  pages={1--23},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{cabrera2021discovering,
  title={Discovering and validating ai errors with crowdsourced failure reports},
  author={Cabrera, {\'A}ngel Alexander and Druck, Abraham J and Hong, Jason I and Perer, Adam},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={5},
  number={CSCW2},
  pages={1--22},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{lee2019webuildai,
  title={WeBuildAI: Participatory framework for algorithmic governance},
  author={Lee, Min Kyung and Kusbit, Daniel and Kahng, Anson and Kim, Ji Tae and Yuan, Xinran and Chan, Allissa and See, Daniel and Noothigattu, Ritesh and Lee, Siheon and Psomas, Alexandros and others},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={3},
  number={CSCW},
  pages={1--35},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@inproceedings{passi2019problem,
  title={Problem formulation and fairness},
  author={Passi, Samir and Barocas, Solon},
  booktitle={Proceedings of the Conference on Fairness, Accountability, and Transparency},
  pages={39--48},
  year={2019}
}

@inproceedings{tanweer2022interrogating,
  title={Interrogating Human-centered Data Science: Taking Stock of Opportunities and Limitations},
  author={Tanweer, Anissa and Aragon, Cecilia R and Muller, Michael and Guha, Shion and Passi, Samir and Neff, Gina and Kogan, Marina},
  booktitle={CHI Conference on Human Factors in Computing Systems Extended Abstracts},
  pages={1--6},
  year={2022}
}

@inproceedings{yang2020towards,
  title={Towards fairer datasets: Filtering and balancing the distribution of the people subtree in the imagenet hierarchy},
  author={Yang, Kaiyu and Qinami, Klint and Fei-Fei, Li and Deng, Jia and Russakovsky, Olga},
  booktitle={Proceedings of the 2020 conference on fairness, accountability, and transparency},
  pages={547--558},
  year={2020}
}



@article{veale2017fairer,
  title={Fairer machine learning in the real world: Mitigating discrimination without collecting sensitive data},
  author={Veale, Michael and Binns, Reuben},
  journal={Big Data \& Society},
  volume={4},
  number={2},
  pages={2053951717743530},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{veale2018fairness,
  title={Fairness and accountability design needs for algorithmic support in high-stakes public sector decision-making},
  author={Veale, Michael and Van Kleek, Max and Binns, Reuben},
  booktitle={Proceedings of the 2018 chi conference on human factors in computing systems},
  pages={1--14},
  year={2018}
}


@inproceedings{holstein2019improving,
  title={Improving fairness in machine learning systems: What do industry practitioners need?},
  author={Holstein, Kenneth and Wortman Vaughan, Jennifer and Daum{\'e} III, Hal and Dudik, Miro and Wallach, Hanna},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--16},
  year={2019}
}

@inproceedings{richardson2021towards,
  title={Towards Fairness in Practice: A Practitioner-Oriented Rubric for Evaluating Fair ML Toolkits},
  author={Richardson, Brianna and Garcia-Gathright, Jean and Way, Samuel F and Thom, Jennifer and Cramer, Henriette},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--13},
  year={2021}
}

@article{lee2020landscape,
  title={The Landscape and Gaps in Open Source Fairness Toolkits},
  author={Lee, Michelle Seng Ah and Singh, Jatinder},
  journal={Available at SSRN},
  year={2020}
}

@article{braun2006using,
  title={Using thematic analysis in psychology},
  author={Braun, Virginia and Clarke, Victoria},
  journal={Qualitative research in psychology},
  volume={3},
  number={2},
  pages={77--101},
  year={2006},
  publisher={Taylor \& Francis}
}

%Creating taxonomy for potential harms
@article{Krger2021HowDC,
  title={How Data Can Be Used Against People: A Classification of Personal Data Misuses},
  author={Jacob Leon Kr{\"o}ger and Milagros Miceli and Florian M{\"u}ller},
  journal={SSRN Electronic Journal},
  year={2021}
}

@article{kaufmann2011more,
  title={More than fun and money. worker motivation in crowdsourcing--a study on mechanical turk},
  author={Kaufmann, Nicolas and Schulze, Thimo and Veit, Daniel},
  year={2011}
}

@article{Buolamwini2019hearing,
  title={More than fun and money. worker motivation in crowdsourcing--a study on mechanical turk},
  author={Kaufmann, Nicolas and Schulze, Thimo and Veit, Daniel},
  year={2011}
}

@article{shen2021everyday,
  title={Everyday algorithm auditing: Understanding the power of everyday users in surfacing harmful algorithmic behaviors},
  author={Shen, Hong and DeVos, Alicia and Eslami, Motahhare and Holstein, Kenneth},
  journal={Proceedings of the ACM on Human-Computer Interaction},
  volume={5},
  number={CSCW2},
  pages={1--29},
  year={2021},
  publisher={ACM New York, NY, USA}
}
@inproceedings{Steiger2021ThePW,
  title={The Psychological Well-Being of Content Moderators},
  author={Miriah Steiger and Timir J. Bharucha and Sukrit Venkatagiri and Martin Johannes Riedl and Matthew Lease},
  year={2021}
}


==> sections/OLD_02_related.tex <==

<Setting up the stage of related>

As companies have been developing responsible AI guidelines and toolkits that incorporate fairness as part of their core values \cite{}, recent years have seen a growing body of work in FAccT and HCI examines the current practice and challenges around AI fairness in industry settings, in order to better support AI fairness practices for industry practitioners (e.g., \cite{}). These works surfaced critical challenges around industry AI fairness practices, including the disconnect between tools offered by the research community versus the actual on-the-ground needs of industry AI practitioners \cite{}, the organizational challenges and barriers around conducting AI fairness work in industry settings \cite{}, and the lack of support around designing appropriate evaluation and amelioration of socio-technical issues raised by AI fairness \cite{}. [A sentence discussing why cross-functional collaboration in fairness/RAI matters, or even just pointing out that there is substantial interdisciplinary work going on in RAI already (with an implicit BUT…) -<In addition, these work suggested that tackling socio-technical issues like AI fairness requires substantial interdisciplinary work done by industry practitioners across roles \cite{}.>


Among all the challeneges, 

\subsection{Cross-functional Collaboration in Industry AI Teams}

Successfully designing, developing, and monitoring AI products and services requires effective communication and collaboration among a diverse range of roles with different disciplinary backgrounds — including software engineers (SWE), data scientists (DS), machine learning (ML) engineers, user experience (UX) designers, product managers (PM), and subject matter, or domain experts (SMEs)\footnote{In Section \ref{4}, we use these acronyms to describe participants' roles.} \cite{amershi2019software, zhang2020data}. Following the norms in industry settings \cite[cf.][]{rakova2021responsible, Henke1993CrossFunctionalTG, song1997cross, kahn1996interdepartmental}, we use the term ``cross-functional collaboration'' to describe the overall communication and collaboration process among these interdisciplinary roles. Prior work studying cross-functional AI collaboration has largely focused on how team members bridge gaps in disciplinary knowledge \cite{piorkowski2021ai, yang2020re, subramonyam2022solving, kross2021orienting, nahar2021collaboration, zhang2020data} and integrate the components of model developing, software engineering, and design throughout the AI product lifecycle \cite{subramonyam2022solving, piorkowski2021ai, nahar2021collaboration, yildirim2022experienced}. For example, Piorkowski et al. [2021] and Kross et al. [2021] surfaced how data scientists leverage different tools and tactics to explain AI concepts to their collaborators with limited or no AI backgrounds \cite{piorkowski2021ai, kross2021orienting}. In another line of work, Yang et al. [2020] and Yildirim et al. [2022] uncovered how designers and UX researchers contribute to the design of AI systems by bringing in end-users' perspectives, while struggling with the lack of a common language when communicating with technical roles on the team \cite{yang2020re, yildirim2022experienced}. Focusing on the collaboration process between UX designers and engineers, Subramonyam et al. [2022] highlighted how designing and building AI systems raised new communication and collaboration challenges on top of the conventional software development \cite{subramonyam2022solving}. 

Although this work focused on cross-functional collaboration for AI development more broadly, some of this prior work has begun to surface collaboration challenges specific to AI fairness efforts \cite{zhang2020data, almahmoud2021teams, nahar2021collaboration}. In our next section, we draw on prior literature in FAccT, Human-Computer Interaction (HCI), and Computer Supported Cooperative Work (CSCW) to better understand the challenges around cross-functional collaboration on fairness in AI.

\subsection{Challenges in Cross-functional Collaboration for AI Fairness in Industry Practice}

A growing body of ethnographic, interview, and co-design studies in FAccT, HCI, and CSCW has examined the current practices and challenges around addressing issues of fairness and responsible AI during design and development of AI systems (e.g., \cite{cramer2018assessing, passi2018trust, passi2019problem, holstein2019improving, madaio2020co, rakova2021responsible, madaio2022assessing, lee2021landscape, richardson2021towards, deng2022exploring, deng2022understanding, wang2023designing, smith2022real}). This work has suggested that appropriately tackling socio-technical issues like AI fairness requires substantial interdisciplinary work done by industry practitioners across roles \cite{passi2019problem, holstein2019improving, madaio2020co, rakova2021responsible, deng2022exploring}. For example, through ethnographic fieldwork with a corporate data science team, Passi and Jackson [2018] highlighted that, in order to build more responsible and trustworthy AI systems, data scientists need to engaging and negotiating with business and product teams throughout the AI developing lifecycle  \cite{passi2018trust}. Rakova et al. [2021] suggested that appropriately tackling AI fairness issue required AI developers to better understand real-world stakeholders' needs through close collaborations with other stakeholders in the organization (e.g., domain experts and legal teams) \cite{rakova2021responsible}. While highlighting the significance around cross-functional collaboration on AI fairness, this work also started to surface related challenges exhibited in the cross-functional collaboration in AI fairness. 

Multiple prior work surfaced that the metrics or methods one discipline uses to evaluate and address AI fairness issues may not be the same as the others, or might even be incommensurate, causing communication breakdown and ineffective collaboration around AI fairness \cite{passi2018trust, passi2019problem, madaio2022assessing, deng2022exploring}. For example, Passi and Barocas [2019] found that the different selections of problem formulations and target proxies between data scientists and business teams could leave AI fairness issue unaddressed at the problem formulation, affecting the quality of downstream AI fairness phase\cite{passi2019problem}. More recently, Madaio et al. [2022] suggests that, practitioners across roles often ``decided to use the same performance metrics that they already used to assess the aggregate performance of their AI systems'' to evaluate the AI fairness for disaggregated subgroups, causing challenges in collectively deciding the most appropriate performance metrics to assess AI fairness \cite{madaio2022assessing}.

Furthermore, existing tools and processes designed for tackling AI fairness issues (e.g., \cite{AIF360API}, \cite{FairlearnAPI}) often only support technical roles working in silo, instead of helping team members with diverse roles draw from each others' expertise and perspectives around AI fairness \cite{deng2022exploring, almahmoud2021teams, lee2021landscape, zhang2020data}. For example, in their work studying how ML practitioners use fairness toolkits to assess and mitigate potential algorithmic biases, Deng et al. [2022] found that data scientists lack efficient tools and processes to communicate with domain experts, making it difficult for them to conduct fairness analyses that drew on domain knowledge \cite{deng2022exploring}. When studying how teams communicate about and evaluate the quality of ML models, Almahmoud et al. [2021] found that product managers attempted to discuss the fairness of models as part of the core model quality, but ``current tools and practices make discussing fairness challenging” as they are often tailored to evaluate and report model qualities like accuracy rather than broader sociotechnical concepts such as fairness \cite{almahmoud2021teams}. Prior work also indicated that there were significant knowledge gaps around AI fairness among AI teams that raised challenges around effective communication and collaboration; The steep learning curve of current AI fairness toolkits and lack of accessible educational resources further added challenges to bridge the knowledge gaps among roles \cite{deng2022exploring, lee2021landscape, richardson2021towards}. 

%Third, the knowledge gaps around AI fairness raised challenges around effective communication and collaboration for the AI teams. Because AI fairness is an emergent and rapidly evolving research field, AI practitioners across roles often lack fundamental knowledge around AI fairness.  \cite{lee2021landscape, deng2022exploring, holstein2019improving}. In addition, effectively collaborating AI fairness around specific applications and regions often required an in-depth domain knowledge around the definition, evaluation, and potential mitigation of algorithmic biases \cite{passi2018trust, Passi2020MakingDS, sambasivan2021re}. The steep learning curve of current AI fairness toolkits and lack of accessible educational resources further added challenges to bridge the knowledge gaps among roles \cite{deng2022exploring, lee2021landscape, richardson2021towards}. 

%Potentially condense this paragraph --- high level description of what they find.
Some literature started to suggested that organizations and many roles on the AI teams often lack awareness or incentivizations to collaborate around AI fairness, often due to the deprioritization of AI fairness in the organization. As Nahar et al. [2022] pointed out, there was significant lack of awareness around fairness in the collaboration between software-engineers and data scientists, and that ``model teams usually do not feel responsible for testing latency, memory consumption, or fairness” \cite{nahar2021collaboration}. Similarly, Zhang et al. found that  \textit{``the assessment and mitigation of bias appears to be treated largely as a technical matter.''} As a result, people ``who may know the most about policy requirements and worry the most about the negative consequences of a biased AI algorithm’’ were often left out of the process of this fairness work \cite{zhang2020data}. 

%Zhang et al. [2020] observed that, though documentation was an important process in the collaboration in AI developments to facilitate the knowledge transfer and version control, because the organization are treating bias mitigation as the most important issue, there was a surprising lack of documentation around the topic of fairness, causing AI fairness issues being unsolved or deprioritized \cite{zhang2020data}. In addition, Zhang et al. found that  \textit{``the assessment and mitigation of bias appears to be treated largely as a technical matter.''} As a result, people ``who may know the most about policy requirements and worry the most about the negative consequences of a biased AI algorithm’’ were often left out of the process of this fairness work \cite{zhang2020data}. 

While prior work provides initial evidence that there exist significant challenges for industry AI practitioners in collaborating on AI fairness, our work extend the prior literature by uncovering how practitioners on cross-functional teams attempt to overcome these challenges, and shed light on the opportunities to better support cross-functional collaboration on AI fairness.









%critical challenges around industry AI fairness practices, including the disconnect between tools offered by the research community versus the actual on-the-ground needs of industry AI practitioners \cite{cramer2018assessing, holstein2019improving, rakova2021responsible}, the organizational challenges and barriers around conducting AI fairness work in industry settings, and how organizational culture shapes AI fairness practices \cite{passi2019problem, madaio2020co, deng2022understanding}, and the lack of support around assessing and mitigating issues of AI fairness
%of socio-technical issues raised by AI fairness 
%\cite{madaio2022assessing, richardson2021towards, deng2022exploring}. 

==> sections/OLD_05_dis.tex <==

As one reason for the current fairness efforts being under recognized was because team members often does not understand (See \ref{invisible_labor}), aligning with Yildirim's call on offering proper education and 




% How do the tactics in our paper diff

Prior work has offered initial evidence for the significance and challenges of cross functional collaboration in AI fairness. Based on a series of interviews and workshops, we identify existing bridging and piggybacking strategies and practices that practitioners are engaging in to enable and better support cross-functional collaboration. %In particular, the critical yet under-recognized “bridging” efforts that overcome various barriers to cross-functional collaboration around AI fairness, and three types of “piggybacking” tactic that attempts circumvents collaboration barriers by attending to the organizational norms and culture. 
In this section, we first discuss concrete implications of these efforts. We then shed light on how offering training and education for AI practitioners might positively affect the collaboration around AI fairness. We end our discussion by highlighting how public policy might contribute to enabling more effective cross-functional collaboration. 

\subsection{Supporting the invisible labor of collaborating around AI Fairness} \label{supporting_visible}

%Discussion: the sustainability of fairness work: lifecycle... manageable work.. (direct design implication from invisible labor) How do we ameliote the burdensome of doing this work...

As mentioned in throughout our findings, carrying out the efforts of bridging and piggybacking often requires practitioners to go beyond their traditional job description, devote additional time and efforts, and take on emotional burdens. %Indeed, Star and Strauss have described this type of work as ``invisible work.'' \cite{gebru2021datasheets} 


To this end, We argue that it is critical for future researchers to (a) create designated tools and processes to support the critical yet under-recognized bridgingwork %, while currently invisible to team members and organizations in general.

% In particular, as a growing body of recent work have been focusing supporting bi-directional learning and knowledge sharing between technical roles and user-facing roles in the AI development pipeline \cite{}, 

One promising future direction for future FAccT and HCI research is to design tools for knowledge sharing across roles when working on AI fairness. For example, designing interactive interfaces (e.g., interactive model cards \cite{crisan2022interactive}) based on existing widely-adopted documentation by industry (e.g., Model cards \cite{mitchell2019model}, Datasheets \cite{gebru2021datasheets}) could potentially serve as boundary objects to facilitate practitioners with diverse backgrounds contribute to the AI fairness efforts. Furthermore, researchers might explore more accessible visualization design to better support practitioners' bridging efforts on cross-disciplinary communication about AI fairness analysis result \cite{deng2022exploring, shen2020designing}. In addition, researchers should also explore new tools and processes to support user-facing roles better communicate contextualized, nuanced fairness notions to technical roles. \dhw{TODO: add specific type of features and design ideas}. For example, researchers could explore building interface \cite{}


As a large amount of effort was spent on navigating the mismatched goals for evaluations of AI fairness from different disciplines, researchers could explore better mechanisms to support mixed-methods approach to evaluate and measure AI fairness. For example, designers and researchers could explore building guidelines and tools to guide AI practitioners to align and complement the insights from quantitative results from data analysis (statistical disparity \cite{} for certain subgroups) and qualitative data from user research (certain subgroup users repeatedly perceived harms and biases) could support the ``co-evaluation'' meetings surfaced in our finding (Section \ref{evaluation}). In addition, researchers ought to think about how to better support translating the evaluation results into the actionable steps that are both technically feasible and encompass the socio-technical nuances in AI fairness, to avoid compromising the values of conducting AI fairness work (Section \ref{quantification}). 

Importantly, in light of the long tradition of participatory design to support workers \cite{muller1993participatory}, we recommend future researchers and companies co-design such tools and processes between researchers and practitioners in order to build tools and processes that attend to practitioners' day to day work.



In contrast to Zhang et al. [2020]'s finding around lack of documentation in collaborations around AI fairness, our finding surfaced that participants from both technical roles (DS) and user-facing roles (UX) using documentation to (Section \ref{contextualization}). 

Future work could explore interfaces that help 

Frameworks, taxonomies, and guidelines providing scaffold on how to connect with (often technical) AI fairness concepts (fairness metrics \cite{}, fairness mitigation algorithm \cite{}, ) to specific application domains . Recent works like <some recent works>

Though the challenges and effort required in producing AI fairness analysis that are accessible to industry practitioners across roles were recently studied in FAccT literature, our finding suggests that these challenges and efforts are still not visible to industry teams \ref{invisible_labor}. This findings draw parallels with Kross and Guo's observations around data scientists' data cleaning and analysis labor being ``magical'' and ``invisible'' to domain experts \cite{kross2021orienting}. Echoing with Kross and Guo's call on changing organizational culture and reward systems to support the ``social-emotional infrastructure'' of data scientists' ``invisible labor'' in their communication with domain experts \cite{kross2021orienting}, we also urge companies proactively recognize and reward the critical invisible labor that enables cross-functional collaboration in AI fairness. One concrete way to implement this is to include the time and efforts devoted to these invisible labor as part of the main KPI, and design organizational OKRs around 
in order to acknowledge the work and make the collaboration efforts sustainable.

Having the key decision makers about designing the KPI, setting up the deadlines, allocating resources, to have realistic expectations of fairness work*** 

- better communicate /through training: help other understand: set up the realistic expectation of what goes into the; important for other team members and managers who have a key to 
For example, <more ideas>

% Disapponting rare how data scientist team... 


% For companies, we argue the first and foremost change is around redesigning the organizational metrics like KPIs. The redesign of organizational KPIs will help recognize the tremendous efforts from practitioners who are currently motivated to conduct AI fairness work, at the same time incentivize team members who are not motivated to do AI fairness work to be more willing to put efforts into the AI fairness efforts, potentially addressing the remaining challenges perceived by practitioners caused by mismatched incentivization \ref{4.3.3}. Importantly, different organizations (or different AI teams within an organization) will have different development cultures and norms. %Our work surfaces practices and tactics our participants adopted as an important step towards better support cross-functional collaboration for AI fairness in industry settings, 

% Some opening around surfacing the invisible work
We see a growing body of work investigating the ``invisible work''
As Wang et al. [2023] shared how UX practitioners adapt their practice to meet responsible AI challenges, collaborating, negotiating, and (sometimes) pushing back technical roles in the design and development process; Kross and Guo [2022] called for the lens of ``data scientist as designers'' and ``sociol-emotional infrastutre'' to better support data scientists navigate the ambiguity and emotional labor when collaborating with clients with domain knowledge \cite{}. Our finding also shed light on the critical  ``bridging'' and ``piggybacking'' work that carry out the collaboration around AI fairness, yet invisible to the organization. To this end, the first and foremost implications 


\dhw{This paragraph is engaging Wong's soft resistance vs. our participants' piggybacking}
Wong [2021] surfaced how UX practitioners use ``soft resistance'' as a powerful tactics to ``make values relevant to other organizational stakeholders,'' or even ``change organizational processes and values.'' \cite{wong2021tactics} However, in our study, we observed AI practitioners' efforts mainly around ``making values relevant'' through ``piggybacking,'' but in their current practice, they stopped there without the attempt to change, even with the vision and hope <......> \dhw{finish this} \ref{}





%We thus hope that these training and education particularly tailored towards AI fairness collaboration could sensitize future industry practitioners about the current invisible labors exhibited in collaboration efforts, ameliorating the frustration and feeling of doing unthankful work for AI fairness practitioners.

%On the other hand, our finding also demonstrate the importance of developing the socio-emotional skills around coping with less motivated team members, especially under the time and resource constraints in carrying out the AI fairness practices \cite{}. 

%Similar to Kross & Guo's call for teaching data scientist socio-emotional skills for communicating with clients, we believe preparing future AI fairness practitioners with strategies to 




\subsection{Aligning the incentivizations of different team members for doing AI Fairness work} \label{aligning}

% How to better align the incentivization from different roles...? With regualation.

%Moreover, as prior research surfaced the potentially comprised nature of conducting AI fairness work in industry setting \cite{madaio2022assessing, rakova2021responsible, deng2022understanding}, our findings reveal participants’ concerns around how the compromised nature of collaboration strategies might fall short of supporting cross-functional collaboration in AI fairness (and AI fairness efforts in general) (Section \ref{4.2}). For example, participants shared concerns about the breakdown of collaboration when piggybacking on business goals is not sufficient as prioritizing fairness contradicts the business goal of profit-driven companies (Section \ref{4.2.2}), along with the perceived frustration due to the discentivizations of doing AI fairness work from other team members. When internal incentivization are insufficient to support more effective collaboration, we argue that regulation and policy from third parties and governments are indispensable in pushing the collaboration happens. While there is an emerging body of policy and regulations (e.g., GDPR \cite{EUdataregulations2018}, AI Bill of Rights \cite{}), these regulations are often being critiqued for lack of teeth towards private companies \cite{}. To this end, future work is much needed to implement policies and regulations that could enforce organization-level awareness and prioritization of AI fairness. It is our hope that these external regulations could strengthen the AI fairness practitioners' efforts to carry on the collaboration across roles.

As shared in Section \ref{invisible_labor}, participants

To make the collaboration around AI fairness and the outcomes of these collaboration more sustainable, 

closely related to the advocate or activist identity described by Chivukula et al. [2022]. 

As mentioned in Section \ref{privacy}, because of the increasingly matured external regulations around privacy, there was a high awareness around privacy and an institutionalized procedure to address potential privacy issues for product teams across their organizations. 


- Building frameworks and tools that help practitioners make a business case for value of doing AI fairness work (similar to the ``soft tactics'' described in Wong [2021] \cite{wong2021tactics}

Iterative nature of Fairness

The rhetorical of Checklist.. 

Invisible labor: need to communicate the boundary... 

documentation showing the labor. (work behind the final results)


\subsection{Re-imagining the training and education of AI practitioners to better prepare them for collaboration on AI fairness} \label{education}

%Our findings uncovered cross-functional collaboration efforts that were critical to push forward AI fairness work yet under-recognized by team members and organizations. 
Many of the issues we identified in this paper arose from a lack of knowledge about AI fairness concepts (as discussed by prior research in the context of using fairness toolkits \cite{lee2021landscape, richardson2021towards, deng2022exploring}), but also largely arose from a lack of understanding of what fairness work involves in practice. %and the tremendous efforts go into facilitating activities and translating domain knowledge (Section \ref{4.1} and \ref{4.3}). 
To this end, we argue that training and education for fairness in AI needs to not only include the knowledge of the technical perspective of AI fairness (e.g., fairness metrics, using fairness toolkits), but also to provide guidance and opportunities for students (or other learners) to  collaborate on AI fairness related projects with learners from other across disciplinary backgrounds, to prepare them to effectively collaborate in industry settings. These opportunities could be in-class activities that include deliberations and discussions across students (cf., Value Cards \cite{shen2021value}, Timelines \cite{wong2021timelines}). As Yildirim et al. suggested in their prior work, in order to prepare designers to work with data scientists to design AI products and services, HCI education for design students for industry should ``consider providing opportunities for working with students from data science programs.’’ \cite{yildirim2022experienced} we believe that future AI and HCI education ought to offer project-based opportunities for students with AI, design, and UX backgrounds to collaborate on topics related to fairness and responsible AI more broadly. Importantly, this type of training and education could bring awareness to the efforts and labor needed to conduct ``bridging'' work in AI fairness collaboration, as well as set up a realistic expectation of the interdisciplinary nature of AI fairness. 

Our finding also surfaced the frequent burdensome and frustration during the collaboration process, either due to their efforts around pushing forward the collaboration were invisible and unappreciated by the organizations, or due to the ``wicked problem'' nature (\cite{}) of addressing AI fairness as a socio-technical issue \ref{}. While striving to reduce these emotional labor 


%As participants leveraging the existing organizational priorities to piggyback their fairness efforts, future policymakers should implement more rigorous regulations that could force a 



% \subsection{Nothing about us without us: The role and power of users in Cross-functional Collaboration for AI Fairness}

% We talked about X, bring opportunities for Y. 

% Our findings shed little light on these questions... 

% In our finding... we observed that participants repeatedly mentioned <something about users>

% \dhw{below are working in progress}


% Users might collaborate? Domain

% \textbf{Bringing in user's voice to help incentivize team workers and see the value of fairness work...}
% Advocacy from users could serve as another important external level to help facilitate the collaboration on AI fairness. Recent years have seen growing efforts from every user’s collective actions in surfacing biases and harmful behaviors exhibited in AI products and services \cite{shen2021everyday, buolamwini2018gender}. As Wang et al. [2023] highlighted in their work, UX practice should consider re-configuring the roles of ``user'' in responsible AI practice in order to complement ``the limited perspectives of researchers and practitioners involved in AI design.'' \cite{madaio2023designing} How might everyday users’ collective actions and advocacy potentially add leverage to the internal cross-functional collaboration around AI fairness efforts? To this end, future research could explore tools and processes that better support practitioners (especially roles that directly interact with users) to advocate and steer the direction of AI fairness work by bringing in end-users’ feedback and audit reports. Similar to the challenges our work surfaced around mismatched evaluation metrics and processes across disciplines \ref{4.2.3}, when studying how industry practitioners engage everyday users in testing and auditing AI systems, Deng et al. [2023] found similar challenges around overcoming the quantification culture in AI development. Future research should explore how to better augment the quantitative analysis around AI fairness through users' day-to-day interaction with AI systems to contextualize the evaluation of AI fairness.




%Our study focused on studying cross-functional collaboration for improving fairness in AI products and services within organizations. However, we acknowledge that the ultimate goal for effective cross-functional collaboration is to benefit the everyday users --- especially those who are being disproportionately harmed by the AI systems \cite{}. As Charlton famously put --- ``nothing about us without us'' --- what role should users play 


==> sections/OLD_deleted.tex <==

%Something about Private
Related to recent discussions in the FAccT community around the tensions between demographic data collection for fairness evaluations and privacy requirements \cite{Andrus2022DemographicReliantAF, Andrus2020WhatWC}, there remain needs for future research to explore the compatibility of AI fairness and privacy, both through an algorithmic lens \cite[cf.][]{Andrus2020WhatWC} and perspectives from risk management \cite[cf.][]{Andrus2022DemographicReliantAF, Hasan2022AlgorithmicBA}. 
%michael.madaio: Andrus and Villeneueve, 2022 (and their 2021 paper too) would be a good start. They have a really nice explication of the tensions demographic data collection for fairness evaluations and privacy requirements

%\placeholder{Importantly, we do recognize that changing the organizational culture could not only rely on individuals or small groups of internal advocate, especially when some AI fairness efforts (e.g., prioritizing the customers who might not generate most profit) might go against company's business goals. In parallel of prior work's call for the, while making a business case for exploring supporting environmental sustainability }

%\placeholder{Laws, industry standards and regulations, and procedures like third party auditing are indispensable in aligning the internal roles' incentivization around working in AI fairness. Future FAccT scholars and relevant policymakers should explore how to design law, regulations, and auditing procedures that could serve as level for practitioners to navigate the collaboration with other roles when working on AI fairness.}



Maybe this is a good point to talk about education: "At a high level, practices are changing, all disciplines need to consider many things including risk, fairness, bias ... which are currently not part of their education or skill set to get a job. How to respond to this? How to develop better curricula that fosters cross-disciplinary work?

\dhw{I want to end the discussion with something around ``how companies might support cross-functional collaboration'' Potentially also connected to Rida's point around ``who should be accountable for facilitating CFC collab? But I'm also having a hard time coming up with more concrete recommendations.}

\dhw{Comments from Rida that I want to highlight in this last paragraph for discussion: One thing to reflect on in the discussion is a reflection on consequences of  leaving the responsibility to do this kind of work to individual vs providing institutional structural  support i.e. with the former you will inevitably get these issues and also unequal division of labor across roles etc.  

 %also perhaps whether we get almost a stunted form of cross disciplinary collaboration when we just leave it for people to define in ad-hoc ways? not that a top down mandatory approach would be better but there needs to be some consistent common goals within the organizations of what cross disciplinary is why its important and how to do it?}

%- Structuring work around 
%- In other forms of work, there are planned, structured work and resources around collaboration among roles (e.g., Software Engineers and UX designers) to design and build products and systems. 
%- Support for cross-functional collaboration for Privacy. 
%- the path 

%Furthermore, the documentation work afterwards could be arduous and time-consuming (Section \ref{invisible_labor}). Therefore, researchers could also explore 
%
%for knowledge synthesizing and sharing across disciplines. 


% There are also activites to support perspective changing and deliberation across roles. potentially draw inspiration from toolkits like Value Cards \cite{shen2021value} and Timelines \cite{wong2021timelines}) to adopt or create activities to achieve the learning objectives for cross-functional collaboration.
%\michael{I'm not sure that this paragraph is adding much - I think we can cut it, unless we have something more concrete to say here}
%\nur{Maybe this is a good point to talk about education: "At a high level, practices are changing, all disciplines need to consider many things including risk, fairness, bias ... which are currently not part of their education or skill set to get a job. How to respond to this? How to develop better curricula that fosters cross-disciplinary work?}
%Throughout our findings, we observed that practitioners desired better processes to solicit and aggregate feedback from users to support their AI fairness efforts (cf. \cite{wang2023designing, deng2022understanding}). To inform the design of new, practitioner-facing processes and tools, researchers should work closely with practitioners to develop systems that can meet the needs and constraints of real-world contexts. In addition, these efforts could draw upon recent work exploring user interface designs to solicit feedback from end users based on their lived experience and domain knowledge \cite{shen2022model, lam2022end}. %For example, interfaces that , or novel approaches that \dhw{add more details for this}
%Importantly, in light of the long tradition of participatory design to support workers \cite{muller1993participatory}, we recommend future researchers and companies co-design such tools and processes between researchers and practitioners in order to build tools and processes that attend to practitioners' day to day work.


- Discussion deleted sentences.

In addition, researchers could potentially draw inspiration from the ``Github commit'' interface that documents and indicates software engineers' code contributions to design similar ``fairness work commits'' to help practitioners track their work and efforts. %\michael{I'm worried we've fallen into the same trap as our participants - what might be lost when or if we adopt a computational paradigm like GitHub to track sociotechnical fairness work?} \dhw{Ah yeah... I think this was inspired by one of the design fiction done by Richmond Wong before, but the artifact was meant to be more provocative than practical... maybe we should consider deleting or revising this (by not mentioning github, but some more general contribution tracking interfaces?} 



% Introduction before.
For instance, in a study of industry collaboration challenges in building AI systems, Nahar et al. [2022] surfaced the lack of awareness around fairness between software engineers and data scientists \cite{nahar2021collaboration}. In other empirical work, Madaio et al. [2022] found that mismatched expectations for model performance metrics from different roles posed obstacles to collectively conducting fairness assessments (i.e., identifying performance disparities for different demographic groups) \cite{madaio2022assessing}. In their work studying how AI practitioners across roles communicate the quality of AI systems, Almahmoud et al. [2021] found that cross-functional AI teams often neglected fairness as part of the model qualities; product managers in the study reported a lack of tools and process to support discussing fairness as part of the AI system qualities with data scientists \cite{almahmoud2021teams}.



\subsubsection{Piggybacking on business goals} % to attempt to collaborate with roles with different priorities than AI fairness} 
\label{4.2.2}

Participants shared that when conducting AI fairness work, they inevitably had to communicate and collaborate with team members who prioritize other aspects of the AI products and services than AI fairness. As P14 mentioned, \emph{``building more fair AI system is not officially integrated into most of my colleagues’ KPI [Key Performance Indicators]. [...] Without telling them that working on this could help them achieve business goals they actually care about to get some promotion, I doubt they would listen to my plan from the very beginning''} (P14). In other words, collaboration around AI fairness was often hindered due to the mismatched performance indicators and priorities for different roles.

To this end, participants often drew on business logics to initiate and motivate collaboration around fairness work. These business logics include avoiding negative Public Relations (PR), gaining market and user retention, and generating more profit. Multiple participants reported that they deliberately chose a different framing about AI fairness when collaborating with different roles. For example, with team members working in marketing and business development, P7 would integrate fairness issues into projects along with business strategy and financial goals. Specifically, P7 used wording like \emph{``serving customers’ demands,”} \emph{``think more long term market,”} and \emph{``establishing a trustworthy branding’’} in project planning meetings to convince roles like business analysts and product managers that AI fairness is worthwhile to consider. 

However, most participants acknowledged that leveraging business logics to motivate fairness work was a \emph{``compromised strategy that is better than nothing''} (P20) in a way that may only temporarily push forward the work, %collaboration, 
but that would not address the AI fairness issue appropriately without genuine motivation of working on AI fairness from some roles. For example, some participants were worried that this approach might \emph{``speed up the collaboration process just for now''} (P3), but could pose challenges to collaboration processes in the future due to the fundamental lack of long-term, cultural changes and the low prioritization of AI fairness efforts. P14 felt disappointed that team members’ fundamental motivations around doing AI fairness work were to compete in the market with other technical companies and \emph{``whether it sounds like a good PR move’’} (P14).
%\emph{``everyone is still treating fairness like a side hustle''} when
Some participants even shared the moral burden around being \emph{``complicit in the ethics-washing''} (P10) of their organizations when they leveraged business logics to motivate fairness work.




% Supporting ht

\begin{comment}

Despite the tremendous efforts around incentivizing different roles to collaborate on AI fairness, many participants shared that one remaining challenge that hindered their collaboration was the lack of incentivization (or disincentivization) around working on AI fairness. 


%\dhw{one more paragraph about misaligned incentivization}

% ------------------------------------------------------------------------------------



Participants share that one reason their bridging work being constantly under-recognized was the misaligned expec

\emph{``So, to be very honest, in my company. The customer service manager mostly collaborates with the product managers and the PM at the product manager, and also the product designers, and then it trickles down to the engineers, so we come a little at the end of the funnel so we don't directly actually come in contact with the users.”}

Because \emph{``as a software engineer, [P16’s] role is how to implement the solution to the problem within the code base, but it's not how to actually solve the problem which the customer is facing,”} P16 reported that their software engineer colleagues \emph{``would love to just code rather than talking to customers, [found P16] weird trying to think more for the users,”} and even {``call[ed] out [P16] for trying to avoid actual work when [P16] was trying to talk to customer services manager,”}. 

As a result, participants believed that companies should expand the \emph{``expectation for what are people supposed to do when working on fairness… especially for our engineering roles (P22)}. In addition, participants shared desire around the redesign of the seasonal evaluation process for employees to make \emph{``individuals’ efforts more implicit and actually tied into the main KPI procedure (P10)”}, to potentially make the invisible labor being recognized and celebrated in the cross-functional collaboration around AI fairness. 


\subsubsection{Burden and Frustration around AI fairness collaboration due to team members’ misaligned incentivizations around AI fairness.}

Participants reported that the invisible labor that was not being recognized in the collaboration work often led to individual’s burn out and frustration that eventually stalled the collaboration process within and across teams. 

% team members perceived/felt. Even in companies with established AI fairness teams, participants still perceived lack of care from coworkers.

Resonating with prior work, participants shared the fact that their team members’ expectations around fairness effort being a one-off improvisation and disengaged right after a single collaboration point. However, participants mentioned that collaboration on AI fairness is not a sprint, but an iterative process that requires thoughtful inputs and long-term care. As a result, multiple participants shared their burden and frustration while collaborating on AI fairness due to the unrealistic expectations that they should \emph{``get the fairness work done so we don’t have to think about it’’ (P14)} For example, P13 shared that some of their colleagues expressed impatience after they attempted to make AI fairness design workshop a standard procedure to run regularly, asking \emph{``did we already do that last time and get the answer?”} 
%Team members and leadership often treated AI fairness (and AI fairness work in general) as an ad-hoc process instead of a standardized procedure. This further affected the design of KPI in the AI development, exacerbating the burden for practitioners devoted themselves to prompting the collaboration around AI fairness.

% Change the discussion around care to incentivization…. "disincentivization" or "de-prioritization"
Participants perceived the organizational lack of care towards AI fairness work also from the ownership of AI fairness work. Because participants were the ones initiating the collaboration around AI fairness, individuals were often treated as \emph{``holding accountable for the fairness work (P7)’’} when the whole company should be responsible for improving fairness in their AI products and services. P2 shared that they felt \emph{``frustrated by the attitude of dodging responsibility for fairness work.”} As a women of color, P2 reported them often felt uncomfortable to \emph{``give everyone a lecture on why fairness should be prioritized."} Furthermore, maintaining the`` bridging” activities often falls onto one or two team members who are highly self-motivated to do the work, but it’s often not sustainable. As P15 told us, \emph{``engineers and data scientists just kind of leave the conversation behind walking out of the meetings you know and I have to spend more time to do most of the work to make sure team can crystallize certain principles or certain best practices.’’} P15 shared the burden towards individuals to maintain the bridging work is not sustainable and frustration around not being able to **** P17 concluded that \emph{``sometimes what got in the way of effective collaboration is not the lack of tools, but lack of care.”}

% while leading the efforts and holding their organizations (and other team members) accountable for building more fair AI products and services. 
% This burden and frustration often constitute emotional labor that affect the effectiveness and sustainability of collaboration efforts.

%As briefly mentioned in \ref{4.1}, conducting ``bridge” activities often require participants to go beyond their traditional job description – technical roles might attempt to initiate conversations with users, and UX designers might spend extra time initiating and organizing co-evaluation sessions to bridge the gaps between quantitative and qualitative evaluations. However, practitioners working on AI fairness repeatedly shared frustration around their coworkers under-recognizing and undermining their efforts and labor. 


\end{comment}
